Towards Counting Markov Equivalence Classes with Logical Constraints

We initiate the study of counting Markov Equivalence Classes (MEC) under logical constraints. MECs are equivalence classes of Directed Acyclic Graphs (DAGs) that encode the same conditional independence structure among the random variables of a DAG model. Observational data can only allow to infer a DAG model up to Markov Equivalence. However, Markov equivalent DAGs can represent different causal structures, potentially super-exponentially many. Hence, understanding MECs combinatorially is critical to understanding the complexity of causal inference. In this paper, we focus on analysing MECs of size one, with logical constraints on the graph topology. We provide a polynomial-time algorithm (w.r.t. the number of nodes) for enumerating essential DAGs (the only members of an MEC of size one) with arbitrary logical constraints expressed in first-order logic with two variables and counting quantifiers (C^2). Our work brings together recent developments in tractable first-order model counting and combinatorics of MECs.

==> Thesis-chapter.tex <==
\chapter{WFOMC with Essential DAG Axiom}\label{ch: essential}

This is an additional chapter providing an idea for WFOMC with \emph{essential DAG axiom}. As usual, it starts presenting an algorithm for counting essential DAGs, and then shows a way to extends it for WFOMC. Although the algorithm for counting essential DAGs is almost as simple as the one for counting DAGs in \cref{sec: DAG_Count}, it was more difficult to make it into a WFOMC algorithm, and the result is way less efficient. Moreover, in order to have domain-liftability, we need to impose a fixed upper bound on the indegree of the nodes of the essential DAG. %As it is now, we do not consider this approach to be useful for applications, but we report if nonetheless for completeness.
%Because of these drawbacks, at present we do not consider this approach to be useful for applications, but we include it here for the sake of completeness.
Because of these drawbacks, at present we consider this approach only as a partial solution to the problem of lifted inference with essential DAG axiom.

\emph{Essential DAGs} are useful structures in the context of causal learning and Bayesian networks. \emph{Bayesian networks} are common graphical models based on DAGs, and two DAGs are said to be \emph{Markov equivalent} if they determine the same Bayesian network, in the sense that they model the same conditional independences among random variables associated to the nodes. Essential DAGs are DAGs that have the property that they are the unique element in their Markov equivalence class. For a reference, see \cite{andersson_characterization_1997}.

\section{Counting Essential DAGs}

Before presenting a way to count essential DAGs, we need a characterization of them as DAGs with certain structural properties. This is done with the following definition and proposition, for which we refer to \cite{andersson_characterization_1997}.

\begin{definition}[Protected Edge]
    In a DAG, an edge $a \to b$ is \emph{protected} if the the set of parents of $a$ is different from the set of parents of $b$ when $a$ is excluded. In other words, $a \to b$ is \emph{not} protected if every parent of $a$ is a parent of $b$ and $b$ has no additional parents apart for $a$.
    %exists a parent of $a$ that is not a parent of $b$, or if there exists a parent of $b$ different from $a$ that is not a parent of $a$.
\end{definition}

\begin{proposition}[\cite{andersson_characterization_1997} Corollary 4.1]
    A DAG is essential if and only if all its edges are protected.
\end{proposition}

By the way, notice that this condition for a DAG to be essential is expressed by the following FOL sentence:
\begin{equation}
    \forall xy. Rxy \to \exists z. (Rzx \land \neg Rzy) \lor (Rzy \land \neg Rzx \land z\neq x)
\end{equation}
where $R/2$ is the relational symbol representing the DAG.
However, the sentence has three variables, so a priori it could be not liftable, and we cannot use it with our WFOMC algorithms.
 
Following \cite{steinsky_enumeration_2003}, let us now derive the recursive formula for counting essential DAGs. This is similar to the one for counting DAGs in \cref{sec: DAG_Count}, but we use sinks instead of sources, because sinks have the following useful property: the DAG obtained removing a sink from an essential DAG is still essential (since the edges remain protected). Hence, we assume the set of nodes to be $[n]$, and for each $i\in [n]$, we let $A_i$ be the set of essential DAGs for which the node $i$ is a sink. Moreover, let $a_n$ denote the number of essential DAGs on $n$ labeled nodes. 
As in \cref{sec: DAG_Count}, the principle of inclusion-exclusion tells us that 
\begin{equation}
    \label{eq:essential_inclusion_exclusion}
    a_n = \Big|\bigcup_{i\in [n]} A_i \Big| = \sum_{m=1}^{n} (-1)^{m+1} \binom{n}{m} |A_{[m]}|
\end{equation}
where $A_{[m]}\coloneqq \cap_{i\in [m]} A_i$.

In order to count $|A_{[m]}|$, we make the following observations, analogous to those in \cref{sec: DAG_Count}:
\begin{remark}\label{observation1_essential}
    If $\omega\in A_{[m]}$, then there are no edges in $\omega$ between the nodes in $[m]$.
\end{remark}
\begin{remark}\label{observation2_essential}
If $\omega\in A_{[m]}$, then the subgraph of $\omega$ restricted to $[\overline m]$ is an essential DAG.
\end{remark}
\begin{remark}\label{observation3_essential}
Because of \cref{observation1_essential}, in order to extend an essential DAG on $[\overline m]$ to an essential DAG in $A_{[m]}$, we can only draw outgoing edges from $[\overline m]$ to $[m]$. Moreover, the outgoing edges that we can draw must be protected. It means that the set of parents of a node $i\in [m]$ can be any subset of $[\overline m]$ that is not made of a node plus exactly its set of parents. Therefore, from the $2^{n-m}$ possible subsets of $[\overline m]$, we need to exclude exactly one subset for each  node in $[\overline m]$, giving $2^{n-m} - (n-m)$ choices for each node $i$ in $[m]$. Thus,  any essential DAG on $[\overline m]$ can be extended to $(2^{n-m} - (n-m))^m$ different essential DAGs in $A_{[m]}$.
\end{remark} 

Since the number of possible essential DAGs on $[m]$ is by definition $a_{n-m}$, \cref{observation3_essential} tells us that there are $(2^{n-m} - (n-m))^m a_{n-m}$ essential DAGs in $A_{[m]}$ that are obtained extending DAGs on $[\overline m]$. But these are all the essential DAGs in  $A_{[m]}$ because of \cref{observation2_essential}, so we conclude that $|A_{[m]}| = (2^{n-m} - (n-m))^m a_{n-m}$. Substituting this value into \cref{eq:essential_inclusion_exclusion} gives the recursive formula we wanted:
\begin{equation}
    \label{eq:counting_essential_DAGs}
    a_n = \sum_{m=1}^{n} (-1)^{m+1} \binom{n}{m} (2^{n-m} - (n-m))^m a_{n-m}
\end{equation}
where $a_0 = 1$. To conclude, notice that by changing the expression in line 3 of \cref{alg:algorithm_DAG}, one can easily derive an algorithm with polynomial complexity for computing the number of essential DAGs on $n$ nodes. 

%Since every DAG has at least one source, we have that the total number of DAGs $a_n$ must be equal to $|\bigcup_{i\in [n]}A_i|$. Moreover, $A_{J}\coloneqq \bigcap_{j \in J} A_j$ is the set of DAGs on $[n]$ such that all the nodes in $J \subseteq [n]$ have indegree zero, and clearly the cardinality of $A_J$ depends only on the cardinality of $J$, not on the individual elements. Thus, we can assume without loss of generality that $J = [m]$ for some $1 \leq m\leq n$, and we now derive a method for computing $A_{[m]}$.


\section{Counting by Splitting with Essential DAG Axiom}

%Let $\Phi$ be a constant-free first-order logic sentence, possibly containing the binary relation $R$.

As usual we first define the essential DAG axiom, plus an axiom that we need for the principle of inclusion-exclusion, similarly to the sets $A_i$.

\begin{definition}
    \label{def:essential_DAG}
    Let $R/2$ be a relational symbol. We say that an interpretation $\omega$ is a model of $EssentialDAG(R, d)$, and write $\omega \models EssentialDAG(R, d)$, if $\omega_R$ forms an essential DAG and the indegree of its nodes is bounded above by $d$.
    %An interpretation $\omega$ is a model of $\Psi = \Phi \land EssentialDAG(R)$ if and only if $\omega$ is a model of $\Phi$ and $\omega_R$ forms an essential directed acyclic graph.
\end{definition}

\begin{definition}
    \label{def: Psi_m_essential}
    Let $\Psi\coloneqq \Phi \land EssentialDAG(R, d)$, where $\Phi$ is an FOL sentence, and the domain is $[n]$. For any $m\in [n]$, we say that an interpretation $\omega$ is a model of $\Psi_{[m]}$, and write $\omega \models \Psi_{[m]}$, if $\omega$ is a model of $\Psi$ and the domain elements in $[m]$ have zero outdegree (i.e.\ are sinks) in the essential DAG formed by $\omega_R$.
    %For any $1 \leq m \leq n$, $\omega$ is a model of $\Psi_{[m]}$ if and only if $\omega$ is a model of $\Psi$ on $[n]$ and the domain elements in $[m]$ have zero $R$-outdegree. 
\end{definition}

The following proposition gives us useful conditions on what we obtain by restring a model of $\Psi_{[m]}$ to $[m]$ and to $[\overline m]$.

\begin{proposition}
    \label{prop:restriction_[m]_essential}
    Let $\Psi \coloneqq \forall xy. \phi(x,y) \land EssentialDAG(R, d)$ and $\Psi' \coloneqq \forall xy. \phi(x,y) \land \neg R(x,y)$, where $\phi(x,y)$ is quantifier-free. Let the domain be $[n]$, and let $1 \leq m \leq n$. If $\omega$ is a model of $\Psi_{[m]}$,  then $\omega \downarrow [m]  \models \Psi'$ and $\omega \downarrow [\overline{m}]  \models \Psi$. 
\end{proposition}
\begin{proof}
The proof is similar to that of proposition \ref{prop: mapping_1}. The only difference is that we need to notice that a subgraph of an essential DAG obtained excluding some sinks is still essential. %This is because 
\end{proof}

%We want to adapt the proof in \cite{WFOMC_DAGs} to do model counting with $\Psi$. Hence, we use the principle of inclusion exclusion, but this time (as done in \cite{enumeration_essential_DAGs}) considering sinks instead of sources. 

Now we need to count the number of extensions of a model of $\Psi'$ on $[m]$ and a model of $\Psi$ on $[\overline m]$ to a model of $\Psi_{[m]}$ on the whole domain $[n]$.
The main problem is that the number of possible extensions when adding a sink depends on the configuration of edges in the essential DAG on $[\overline m]$: in the algorithm for counting essential DAGs, for each sink in $[m]$ we excluded a subset of $[\overline m]$ for each node in $[\overline m]$; now, the quantity to subtract depends on the graph made by $R$ on $[\overline m]$ and the different $1$-types of the nodes. 

To tackle this, we introduce new predicates $A_{(t_1,\dots,t_u)}/1$ saying \say{a node $y$ has $t_1$ $R$-parents of $1$-type $1$, $t_2$ $R$-parents of $1$-type $2$, ..., $t_u$ $R$-parents of $1$-type $u$}, i.e. satisfying the condition
\begin{equation}
    \label{eq:new_predicates_essential}
    \forall y. A_{(t_1,\dots,t_u)}(y)\leftrightarrow (\exists^{=t_1}x.1(x)\wedge R(x,y))\wedge\dots\wedge (\exists^{=t_u}x.u(x)\wedge R(x,y))
\end{equation}
for any vector of natural numbers $\bt =(t_1,\dots,t_u)$ with $|\bt|\leq d$.
Let us denote by $T$ the set of all such vectors. Since the new predicates are all mutually exclusive, we can reduce the new $1$-types (i.e.\ the ones given the new predicates) to the pairs given by one of the $u$ original $1$-types and by a vector $\bt \in T$. In the following, we use capital letters to index these extended $1$-types, and the cardinality vectors $\bk, \bk', \bk''$ also refer to these extended $1$-types. 

The following proposition  --- analogous to \cref{prop: extensions_k} for DAGs and \cref{prop: extensionsConWeighted} for connected graphs --- gives us a way to calculate the number of extensions to be used for computing $\fomc(\Psi_{[m]}, \bk)$. For simplicity we do not consider weights, but the results can be easily extended for WFOMC (instead of just FOMC).

\begin{proposition}
    \label{prop: extensions_k_essential}
%Let $\Psi \coloneqq \forall xy. \phi(x,y) \land Acyclic(R)$ and $\Psi' \coloneqq \forall xy. \phi(x,y) \land \neg R(x,y)$, where $\phi(x,y)$ is quantifier-free, and let the domain be $[n]$. Let $\omega'$ be a model of $\Psi'$  on the domain $[m]$ and let $\omega''$ be a model of $\Psi$ on the domain $[\overline{m}]$. 
%Then, the weighted sum of the extensions $\omega$ of $\omega' \uplus \omega''$ such that $\omega \models \Psi_{[m]}$ is
%\begin{equation}
%    \label{eq: extensions}
%    \w(\omega') \cdot \w(\omega'') \cdot \prod_{i,j\in[u]} r_{ij}^{k'_i \cdot k''_j} 
%\end{equation}
%where $k'_i$ and $k''_j$ are the number of domain constants realizing the $i^{th}$ and $j^{th}$ $1$-types in $\omega'$ and $\omega''$ respectively; and $r_{ij} \coloneqq \sum_{l \in [b]}n_{ijl}v_l$, where $v_l$ is defined in \cref{eq: v_l} and 
%\begin{align}
%    \label{nijl_bis}
%    n_{ijl} \coloneqq
%    \begin{cases} 
%        1 & \text{if \/ $ijl(x,y) \models \phi(\{x,y\}) \land \neg R(y,x) \land \neg R(x,x) \land \neg R(y,y)$} \\
%        0 & \text{otherwise} \\
%    \end{cases}
%\end{align} 
    Let $\Psi \coloneqq \forall xy. \phi(x,y) \land EssentialDAG(R, d)$ and $\Psi' \coloneqq \forall xy. \phi(x,y) \land \neg R(x,y)$, where $\phi(x,y)$ is quantifier-free, and let the domain be $[n]$. Since DAGs do not admit loops, we also assume without loss of generality that $\phi(\{x,y\}) \models \neg R(x,x)$. Let $\omega'$ be a model of $\Psi'$  on the domain $[m]$ and let $\omega''$ be a model of $\Psi$ on the domain $[\overline{m}]$. Then, the number of extensions $\omega$ of $\omega' \uplus \omega''$  such that $\omega \models \Psi_{[m]}$ is
    \begin{equation}
        \label{eq:extensions_essential}
        N(\phi, \bk', \bk'') \coloneqq \prod_{J\in[u]\times T} \left(
            \left(\prod_{I\in [u]\times T} a_{IJ}^{k''_I}\right) - b_J
        \right)^{k'_J}
    \end{equation}
    where \begin{itemize}
        \item $k'_J$ (resp. $k''_I$) is the number of domain constants realizing the extended $1$-type $J$ (resp. $I$) in $\omega'$ (resp. $\omega''$);
        \item $a_{IJ} \coloneqq \sum_{l \in [b]}a_{IJl}$ and %$a_{IJl}$ is $1$ if $$IJl(x,y) \models \phi(\{x,y\}) \land \neg R(y,x) \land \neg R(x,x) \land \neg R(y,y) \land \cref{eq:new_predicates_essential}$$ and $0$ otherwise;
        \begin{align}
            \label{a_IJl}
            a_{IJl} \coloneqq
            \begin{cases} 
                1 & \text{if \/ $IJl(x,y) \models \phi(\{x,y\}) \land \neg R(y,x) \land \cref{eq:new_predicates_essential}$} \\
                0 & \text{otherwise} \\
            \end{cases}
        \end{align} 
        \item
            \begin{equation}
            \label{eq:b(j,t)}
            b_{(j,\bt)} \coloneqq \left(\sum_{i\in [u] | t_i>0}k''_{(i,\bt^{-i})}
            \sum_{v\in [b]} c_{ijl}\sum_{\bv\in [b]^{|\bt|-1}}\prod_{p=1}^{|\bt|-1} c_{f(p)jv_{p}}\right)
            \prod_{\iota\in [u]} {d}_{\iota j}^{k''^{-\bt}_\iota}
            \end{equation}
       where 
        \begin{itemize}
        \item $\bt^{-i}\coloneqq(t_1,\dots, t_{i-1}, t_i - 1, t_{i+1}, \dots, t_u)$ is $\bt$ minus the vector with $1$ in position $i$ and $0$ in all other positions;
        \item $c_{ijl}$ is $1$ if $ijl(x,y) \models \phi(\{x,y\}) \land \neg R(y,x) \land R(x,y)$, %\land \neg R(x,y) \land \neg R(y,y)$, 
        and $0$ otherwise;
        \item $f$ is a function which enumerates the original $1$-types encoded as units in $\bt$, and $c_{f(p)jv_p}$ is $1$ if $f(p)jv_p(x,y) \models \phi(\{x,y\}) \land \neg R(y,x) \land R(x,y)$ and $0$ otherwise;
        \item $d_{\iota j} \coloneqq \sum_{l \in [b]}d_{\iota jl}$ and $d_{\iota jl}$ is $1$ if $\iota jl(x,y) \models \phi(\{x,y\}) \land \neg R(y,x) \land \neg R(x,y)$, and $0$ otherwise;
        \item $\bk''^{-\bt}$ is the vector of length $u$ obtained summing up the values of $\bk''$ relative to the same original $1$-types, and finally subtracting $\bt$.
    \end{itemize}\end{itemize}
\end{proposition}
\vspace{-4.2em}
\begin{proof}[proof idea]
    First, notice that we can treat the sinks in $[m]$ independently, and for each one we simply have to ensure that the $R$-edges arriving to them are protected. So, for each extended $1$-type $J$ for a sink in $[m]$, we first count all the possible ways to interpret the binary relations concerning such a node and the nodes in $[\overline m]$, possibly forming unprotected $R$-edges. Analogously to the proof of \cref{prop: extensions_k}, this is given by $\prod_{I\in [u]\times T} a_{IJ}^{k''_I}$.  From this we have to subtract $b_J$, which counts the number of ways in which there can be an unprotected $R$-edge to such node. Then, considering independently the sinks in $[m]$ with all their extended $1$-types $J$ encoded in the $1$-types cardinality vector $\bk'$, we get \cref{eq:extensions_essential}. %This explains \cref{eq:extensions_essential}, and notice that we needed the extended $1$-types because they are useful for the induction.

    It remains to be shown how to derive the formula for $b_{J}$ (or $b_{(j,\bt)}$) given in eq.\ \eqref{eq:b(j,t)}. With $\bt$, we have fixed the (original) $1$-types of the $R$-parents of a sink we are considering (and in particular its number of $R$-parents $|\bt|$). We need to count all the cases in which one of the parents is a child of exactly all the rest. Notice that such a node which is child of all the rest needs to have an extended $1$-type $(i,\bt^{-i})$ for an $i\in [u]$ such that $t_i>0$. This gives us the first summation and the factor $k''_{(i,\bt^{-i})}$ counting how many nodes can be found with each extended $1$-type. Indeed, it can be proven that a node cannot have more than one unprotected edge to it, so the possibilities are mutually exclusive and can be simply summed up. 

    Then we need to count the ways to connect a node of extended $1$-type $(i,\bt^{-i})$, and its parents, to the sink of extended $1$-type $(j,\bt)$. This is given by the term
    \[
        \sum_{v\in [b]} c_{ijl}\sum_{\bv\in [b]^{|\bt|-1}}\prod_{p=1}^{|\bt|-1} c_{f(p)jv_{p}}    
    \]
    because for each possible $2$-table for each $R$-parent of the sink, we just need to ensure that there is an $R$-edge going from the $R$-parent to the sink. Requiring such $R$-edges is done by multiplying $c_{ijl}$ (for the node that is a child of the rest) and all the $c_{f(p)jv_{p}}$ (for the rest of the parents); then we need to sum over all the different possibilities for the $2$-tables.

    Finally, we need to count the extensions for the other nodes, those which are not $R$-parents of the sink we are considering. In particular, the condition of not being $R$-parents is encoded by $d_{\iota j}$ and the cardinalities of such nodes for each (original) $1$-type are encoded by $\bk''^{-\bt}$. Since the ways to extend in this case are independent from each other and from the nodes previously considered as parents, we get the last product in formula \eqref{eq:b(j,t)}.
\end{proof}

The previous proposition was the tricky part; now the remaining is as in \cref{sec: WFOMC_DAGs}.

\begin{proposition}\label{prop:induction_essential}
    Let $\Psi \coloneqq \forall xy. \phi(x,y) \land EssentialDAG(R, d)$ and $\Psi' \coloneqq \forall xy. \phi(x,y) \land \neg R(x,y)$, where $\phi(x,y)$ is quantifier-free. Then:     
    \begin{equation}
        \label{eq: k_k'_m_essential}
        \fomc(\Psi_{[m]},\bk) =
        \sum_{\substack{\bk= \bk'+\bk''\\ |\bk'|=m}} N(\phi, \bk', \bk'') \cdot \fomc(\Psi',\bk')\cdot\fomc(\Psi,\bk'' )
    \end{equation}
    %where $\bk'+\bk''$ represents the element-wise sum of integer-vectors $\bk'$ and $\bk''$, such that $|\bk'|=m$ and $|\bk''| = |\bk|-m$.
    where $N(\phi, \bk', \bk'')$ is defined in \cref{prop: extensions_k_essential}.
\end{proposition}
\begin{proof}
    Similar to the proof of \cref{prop: atleast_weighted}. What changes is the number of extensions $N(\phi, \bk', \bk'')$, which is computed with the previous proposition.
\end{proof}


\begin{proposition}
    Let $\Psi \coloneqq \forall xy. \phi(x,y) \land EssentialDAG(R,d)$, where $\phi(x,y)$ is quantifier-free. Then:
    %The first order model count of the formula $\Psi = \forall xy. \Phi(x,y) \land EssentialDAG(R)$ is given as:
    \begin{equation}
        \label{eq: DAG_Acyclic_essential}
        \fomc(\Psi ,\bk) = \sum_{m=1}^{n}(-1)^{m + 1}\binom{|\bk|}{m}\fomc(\Psi_{[m]},\bk)
    \end{equation} 
\end{proposition}
\begin{proof}
    Similar to the proof of \cref{prop:final_acyclic}. What changes is the definition of the sets $A_i$, as the sets of models $\omega$ such that $\omega\models \Psi \land \bk$ and the domain element $i$ is a sink in $\omega_R$.
\end{proof}

From this, one could derive an algorithm with polynomial complexity for WFOMC with the axiom $EssentialDAG(R,d)$, similar to the ones presented in the previous chapters. However, %notice how impractical it is, given the new $1$-types.
beside the difficulty of \cref{prop: extensions_k_essential},
recall that the algorithmic complexity is exponential in the number of $1$-types, and we are augmenting the number of $1$-types from $u$ to something approximately in the order of $u^d$. So, a WFOMC algorithm for essential DAGs following this approach would be much worse that the one for DAGs in \cref{sec: WFOMC_DAGs}.%, that already did not scale so well according to the experiments in \cref{ch: experiments}.



\begin{comment}
\section{Counting Essential DAGs by Indegree}

Let's derive the formula for counting essential DAGs from the one for FOMC with the essential DAG axiom.

In order to do so, we consider the case in which $\Phi = \top$ and there is only the binary relation $R$ and no other predicate. In particular, there are only two $1$-types (namely $R(x,x)$ and $\neg R(x,x)$), of which $\neg R(x,x)$ is always satisfied (since DAGs have no self-loops). This means that we can consider as if it were $u=1$, and the extended $1$-types were given just by the number $|\bt|$ (but let us call it just $t$) of parents of a node. Hence, we can read the vector $\bk$ as a vector of length $d$ such that $k_t$ specifies how many nodes have in-degree $t$, for each $t=1,\dots,d$. The same for $\bk'$ and $\bk''$, with the difference that they refer to a subset of the nodes ($[m]$ for $\bk'$ and $[\overline m]$ for $\bk''$).

Now, the two tables are $R(x,y) \land \neg R(y,x)$, $R(y,x) \land \neg R(x,y)$, $\neg R(x,y) \land \neg R(y,x)$ and $R(x,y) \land R(y,x)$, of which the last is never satisfied because of the acyclicity axiom. Hence $a_{IJl}$ is $1$ for $l=R(x,y) \land \neg R(y,x)$ and for $l=\neg R(x,y) \land \neg R(y,x)$, and $0$ otherwise (irregardless of $I$ and $J$). This makes $a_{IJ}=2$ for any $I,J \in T$.

Now, let us compute $b_J$, or better $b_t$ (since we have explained how extended $1$-types are now represented by a single number). The first summation in formula \ref{eq:b(j,t)} is on a single value, so it is no more an actual summation. Then, we notice that for $c_{ijl}$ to be $1$ we need $v=\neg R(y,x) \land R(x,y)$, giving just one possibility for $v$ (irregardless of $i$ and $j$). The same for $c_{f(p)jv_p}$, for each $v_p$. Thus, also the other summations are on a single value (the others being $0$), and the quantity between brackets is simply $k''_{t-1}$. Finally, $d_{\iota jl}$ is $1$ iff $l=\neg R(x,y) \land \neg R(y,x)$, leaving again only one possibility. So, $d_{\iota j}=1$ and the whole product is $1$. 

In conclusion, we have shown that in our case
\begin{equation}
    \label{eq:sanity_check1}
    N(\top, \bk', \bk'') = \prod_{t=0}^d \left( \prod_{t'=0}^d 2^{k''_{t'}} - k''_{t-1}\right)^{k'_{t}} = \prod_{t=0}^d \left(2^{|k''|} - k''_{t-1}\right)^{k'_{t}}
\end{equation}

Now that we have analyzed \cref{prop: extensions_k_essential} we can pass to \cref{prop:induction_essential}. In this setting, $\fomc(\Psi_{[m]},\bk)$ is the number of essential DAGs on the nodes $[n]$ such that the nodes $[m]$ are terminal and the number of nodes with in-degree $t$ is given by $k_t$. Moreover, $\fomc(\Psi',\bk')=1$, since the only way to satisfy $\Psi'$ is that no arrows are drawn. This leaves us with 
the formula 
\begin{equation}
    \label{eq:sanity_check2}
    \fomc(\Psi_{[m]},\bk) = \sum_{\substack{\bk= \bk'+\bk''\\ |\bk'|=m}}\prod_{t=0}^d \left(2^{n-m} - k''_{t-1}\right)^{k'_{t}} \cdot \fomc(\Psi,\bk'')
\end{equation}
%and finally
%\begin{equation}
%    \label{eq:sanitycheck3}
%    \fomc(\Psi ,\bk) = \sum_{m=1}^{n}(-1)^{m + 1}\binom{|\bk|}{m} \sum_{\substack{\bk= \bk'+\bk''\\ |\bk'|=m}}\prod_{t=0}^d \left(2^{n-m} - k''_{t-1}\right)^{k'_{t}} \cdot \fomc(\Psi,\bk'')
%\end{equation} 
which can be substituted inside \cref{eq: DAG_Acyclic_essential} to get the final recursive formula.
%\[
%\sum_{|\bk|=n}\fomc(\Psi_{[m]},\bk) = \sum_{|\bk'|=m}  \sum_{|\bk''|=n-m} \prod_{t=0}^d \left(2^{n-m} - k''_{t-1}\right)^{k'_{t}} \cdot \fomc(\Psi,\bk'')
%\]
Even if it is not the formula in \cite{enumeration_essential_DAGs}, it makes sense. Indeed it is a similar formula that takes into account the number of nodes with each possible in-degree provided with vector $\bk$. It can be proven with the same idea from \cite{enumeration_essential_DAGs}, just taking into account $\bk$. Notice that to get the number of all possible essential DAGs with $n$ nodes we simply have to sum over the possible vectors $\bk$.
\end{comment}
